On M-ary Distributed Detection for Power Constraint Wireless Sensor Networks

We consider a wireless sensor network (WSN), consisting of several sensors and a fusion center (FC), which is tasked with solving an M-ary hypothesis testing problem. Sensors make M-ary decisions and transmit their digitally modulated decisions over orthogonal channels, which are subject to Rayleigh fading and noise, to the FC. Adopting Bayesian optimality criterion, we consider training and non-training based distributed detection systems and investigate the effect of imperfect channel state information (CSI) on the optimal maximum a posteriori probability (MAP) fusion rules and optimal power allocation between sensors, when the sum of training and data symbol transmit powers is fixed. We consider J-divergence criteria to do power allocation between sensors. The theoretical results show that J-divergence for coherent reception will be maximized if total training power be half of total power, however for non coherent reception, optimal training power which maximize J-divergence is zero. The simulated results also show that probability of error will be minimized if training power be half of total power for coherent reception and zero for non coherent reception.

==> README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> figure.tex <==
%\newpage
\newcommand\invisiblesection[figure]{%
  \refstepcounter{section}%
  \addcontentsline{toc}{section}{\protect\numberline{\thesection}#figure}%
  \sectionmark{#figure}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_clos_bin_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_clos_bin_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_clos_bin_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=2$, $N=5$ and sensors closer to FC perform better.i) Coherent reception ii) Non-coherent reception with amplitude estimation iii) Non-coherent reception with channel statistic.}
                 \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!hbp]
        \centering
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_clos_bin_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iv)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_clos_bin_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(v)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_clos_bin_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(vi)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=2$, $N=5$ and sensors closer to FC perform better. i) Coherent reception ii) Non-coherent reception with amplitude estimation iii) Non-coherent reception with channel statistic.}
                \end{figure*}
                
          
        % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
        \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_clos_4ary_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_clos_4ary_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_clos_4ary_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_clos_4ary_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iv)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_clos_4ary_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(v)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_clos_4ary_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(vi)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=4$ and different receptions when sensors closer to FC perform better, in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10.}
                \end{figure*}
                
          
        % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_far_bin_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_far_bin_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_far_bin_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_far_bin_10.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_far_bin_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_far_bin_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=2$ and different receptions when sensors farther from FC perform better, in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10.}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                 % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_far_4ary_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_far_4ary_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_far_4ary_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_far_4ary_10.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_far_4ary_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_far_4ary_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=4$ and different receptions when sensors farther from FC perform better, in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10.}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqdist_bin_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqdist_bin_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqdist_bin_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqdist_bin_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iv)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqdist_bin_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(v)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqdist_bin_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(vi)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=2$ and different receptions when sensors are situated in equal distance from FC with different performance,in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10.}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqdist_4ary_5.pdf}
          
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqdist_4ary_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqdist_4ary_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqdist_4ary_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iv)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqdist_4ary_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(v)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqdist_4ary_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(vi)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=4$ and different receptions when sensors are situated in equal distance from FC with different performance,in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10.}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqperf_bin_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqperf_bin_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqperf_bin_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqperf_bin_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iv)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqperf_bin_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(v)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqperf_bin_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(vi)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=2$ and different receptions when sensors have equal performance but in different distance from  cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10., in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10..}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqperf_4ary_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqperf_4ary_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqperf_4ary_5.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(iii)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqperf_4ary_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iv)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!htbp]{0.3\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqperf_4ary_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(v)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        \begin{minipage}[!htbp]{0.3\textwidth}
                  \centering
                  \includegraphics[width=1\textwidth]{stat_eqperf_4ary_10.pdf}
                  \vspace{-0.6cm}
                  %\caption{\footnotesize x1.}
                  \centerline{(vi)}\medskip
                  \label{fig:x1}
                \vspace{0.4cm}
                \end{minipage}
                \caption{Probability of error vs SNR for $M=4$ and different receptions when sensors have equal performance but in different distance from  cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10., in cases (i), (ii),(iii) N=5 and in cases (iv), (v), (vi) N=10..}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_clos_bin_rd_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_clos_bin_rd_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_clos_bin_rd_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iii)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_clos_bin_rd_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(iv)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        
                \caption{Probability of error vs $r_d$ for $M=2$ and different receptions when sensors closer to FC perform better, in cases (i), (ii) N=5 and in cases (iii), (iv) N=10.}
                \end{figure*}
                
          
        % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
        \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_far_bin_rd_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_far_bin_rd_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
       
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_far_bin_rd_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iii)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_far_bin_rd_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(iv)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        
                \caption{Probability of error vs $r_d$ for $M=2$ and different receptions when sensors farther from FC perform better, in cases (i), (ii) N=5 and in cases (iii), (iv) N=10.}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqdist_bin_rd_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqdist_bin_rd_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqdist_bin_rd_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iii)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqdist_bin_rd_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(iv)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        
                \caption{Probability of error vs $r_d$ for $M=2$ and different receptions when sensors are situated in equal distance from FC with different performance, in cases (i), (ii) N=5 and in cases (iii), (iv) N=10.}
                \end{figure*}
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                
                \begin{figure*}[!hbp]
        \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqperf_bin_rd_5.pdf}
          \vspace{-0.6cm}
          \centerline{(i)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqperf_bin_rd_5.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(ii)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
       
                %%%%%%%%%%%%%%%%%%%%%
                 \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{coh_eqperf_bin_rd_10.pdf}
          \vspace{-0.6cm}
          \centerline{(iii)}\medskip
         % \caption{\footnotesize 1.a.}
          %\label{fig:x1}
        \vspace{0.4cm}
        \end{minipage}
          \centering
        \begin{minipage}[!hbp]{0.48\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{non_eqperf_bin_rd_10.pdf}
          \vspace{-0.6cm}
          %\caption{\footnotesize x2.}
          \centerline{(iv)}\medskip
          \label{fig:x2}
        \vspace{0.4cm}
        \end{minipage}
        
                \caption{Probability of error vs $r_d$ for $M=2$ and different receptions when sensors have equal performance but in different distance from FC, in cases (i), (ii) N=5 and in cases (iii), (iv) N=10.}
                \end{figure*}
                
            
       
